Scalable Hypergraph Embedding System

Many problems such as node classification and link prediction in network data can be solved using graph embeddings. However, it is difficult to use graphs to capture non-binary relations such as communities of nodes. These kinds of complex relations are expressed more naturally as hypergraphs. While hypergraphs are a generalization of graphs, state-of-the-art graph embedding techniques are not adequate for solving prediction and classification tasks on large hypergraphs accurately in reasonable time. In this paper, we introduce HyperNetVec, a novel hierarchical framework for scalable unsupervised hypergraph embedding. HyperNetVec exploits shared-memory parallelism and is capable of generating high quality embeddings for real-world hypergraphs with millions of nodes and hyperedges in only a couple of minutes while existing hypergraph systems either fail for such large hypergraphs or may take days to produce the embeddings.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We describe HyperNetVec, a multi-level hypergraph embedding framework, which can process hypergraphs with millions of nodes and hyperedges in just a few minutes, producing high-quality embeddings for node classification and hyperedge prediction. Our experimental results show that it significantly outperforms multi-level graph embedding approaches such as MILE and GraphZoom in both accuracy and running time (some of these approaches fail for the large datasets in our studies). We also showed that our refinement algorithm can be used on its own to improve the quality of embeddings for hypergraphs by up to 23\%.

